A Unified Concept-Based System for Local, Global, and Misclassification Explanations

Explainability of Deep Neural Networks (DNNs) has been garnering increasing attention in recent years. Of the various explainability approaches, concept-based techniques stand out for their ability to utilize human-meaningful concepts instead of focusing solely on individual pixels. However, there is a scarcity of methods that consistently provide both local and global explanations. Moreover, most of the methods have no offer to explain misclassification cases. Considering these challenges, we present a unified concept-based system for unsupervised learning of both local and global concepts. Our primary objective is to uncover the intrinsic concepts underlying each data category by training surrogate explainer networks to estimate the importance of the concepts. Our experimental results substantiated the efficacy of the discovered concepts through diverse quantitative and qualitative assessments, encompassing faithfulness, completeness, and generality. Furthermore, our approach facilitates the explanation of both accurate and erroneous predictions, rendering it a valuable tool for comprehending the characteristics of the target objects and classes.

==> tabels/SSC_SDC_3Methods.tex <==
\setlength{\tabcolsep}{1cm}           % set horizontal space for all column (before and after col)
%remove space with @{}  and change it with @\quad   or  @{\hspace{5cm}}
\renewcommand{\arraystretch}{1}       %vertical space  for all  rows (1.2 times default)
\begin{table}[h!]
% \begin{wraptable}{R}{7.0cm}
		\caption{The values of $\mathrm{SSC}$ and $\mathrm{SDC}$  over all the random samples. } \label{tab:SSC_SDC_5methods}%
	\vskip -0.1in
\begin{center}

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{@{} lcr @{}}
\toprule
         &  $\mathbf{ \mathrm{SSC} (\downarrow)}$  &   $\mathbf{ \mathrm{SDC}(\downarrow)}$ \\
\midrule

LIME     &     13.42     &  \textbf{1.89 }    \\
SHAP      &    9.73     & \textbf{1.19 }    \\
GradCAM      &   18.84      &  2.20    \\
LRP      &   16.68      &  2.03    \\
UCBS      &   \textbf{8.31}     & \textbf{1.60}    \\

 \bottomrule
\end{tabular}%

			
\end{center}
	\vskip -0.1in

\end{table}% 

						
 			
